Optimal Stateless Model Checking of Transactional Programs under Causal Consistency

We present a framework for efficient stateless model checking (SMC) of concurrent programs under five prominent models of causal consistency, CCv,CM,CC, Read Committed and Read Atomic. Our approach is based on exploring traces under the program order (po) and the reads from (rf) relations. Our SMC algorithm is provably optimal in the sense that it explores each po and rf relation exactly once. We have implemented our framework in a tool called TRANCHECKER. Experiments show that TRANCHECKER performs well in detecting anamolies in classical distributed databases benchmarks.

==> ra-rc-denota.tex <==

 \section{Denotational Semantics $\readc, \readat$}
 \label{app:denot}
We give the denotational semantics for the models $\readat, \readc$ which 
were no included in section \ref{sec:tr} due to space constraints. 
 

  \noindent{\bf{Read Committed $\readc$}}. 
 $\readc$ is one of the weakest models for causal consistency \cite{DBLP:conf/sigmod/BerensonBGMOO95}.   Like $\ccvt$, the consistency condition is defined by extending traces with the $\cfr$ relation between transactions writing to the same variable. 
 For transactions $t_1, t_2 \in \tran^{\wt,x}$ for some variable $x$, 
 $t_1~\cfr~t_2$  is defined by ensuring that the  
 corresponding read events  appearing in a transaction $t\in \tran^{\rd,x}$ are \emph{monotonic}. To capture  
   monotonicity between events in a transaction, we use the \emph{transaction order} $\tto$ which orders events within a transaction. If $e_1, e_2, \dots, e_k$ is the ordered sequence  of events in a transaction $t$, define $e_i~\tto~e_j$ for $i < j$. 
   The intuition is that for $e_1, e_2 \in \eventset^{\rtype,t}$ with  $e_1~\tto~e_2$, if $e_1 \in \eventset^{\rtype,\xvar,t}$ reads from a transaction $t_1$, and $e_2 \in \eventset^{\rtype,\yvar, t}$ reads from a transaction $t_2$, and  $t_1, t_2 \in \tran^{\wt,x}$, then 
   $t_2$ must be ''$\cfr$-later'' than $t_1$, that is, $t_1~\cfr~t_2$. 
 That is, for all variables $x$, and all transactions $t_1 \neq t_2 \in \tran^{\wt,x}$, if there exist read events $e_1~\tto~e_2$ in $t \in \tran$ such that  $t_1~\trf~e_1, t_2~\trf~e_2$, then $t_1~\cfr~t_2$.  
       
         \begin{figure}[h]
 	\includegraphics[width=15cm]{prog1.pdf}
 \caption{Differences between consistency models. 
 The \textcolor{blue!80!green}{$\triangleright v$} denotes the expected 
 return value of the read event.  }
 \label{fig:bad-app}
 \end{figure}

       
Define a function $\extend_{\readc}(\tau)$ which extends a trace $\tau=(\tran, \tpo, \trf)$ by 
  adding all possible $\cfr$ edges between transactions  which write on the same variable. 
  In $\extend_{\readc}(\tau)$, we do not draw the $\trf$ edges 
  from transactions $t \in \tran^{\wt,x}$ to read events 
 $e \in \eventset^{\rtype,\xvar, t'}$; these are used to draw the $\cfr$ edges between transactions.     
 Traces violating $\readc$ exhibit a $\tpo \cup \cfr$ cycle in $\extend_{\readc}(\tau)$, which we refer to as a $\readccyc$. We say that $\tau \models \readc$ iff $\extend_{\readc}(\tau)$ does not contain a $\readccyc$. 
%   
% 

\smallskip 

 \noindent{\emph{Examples}}. For the program Fig.\ref{fig:bad-app}(a), and any trace $\tau$, $\extend_{\readc}(\tau)$ contains $\readccyc$. 
  Consider the read events $e_1={\tt{a}}:=y$, $e_2={\tt{b}}:=x$ in $t_4$, 
   such that $e_1~\tto~e_2$ and $t_3~\trf~e_1$, $t_1~\trf~e_2$, with $t_1, t_3 \in \tran^{\wt,x}$. Then we have $t_3~\cfr~t_1$. Likewise, 
   $t_4$ has the read event $e_3={\tt{c}}:=z$ with $e_2~\tto~e_3$. 
   Since $t_2~\trf~e_3$, we obtain $t_1~\cfr~t_2$ resulting in a 
   cycle. Likewise, for the  program Fig.\ref{fig:bad-app}(d), we obtain $t_1~\cfr~t_2$ (reads in $t_5$) as well as $t_3~\cfr~t_1$ (reads in $t_4$).  
%  
%  
 \smallskip 
 
  \noindent{\bf{Read Atomic $\readat$}}. This model \cite{DBLP:conf/concur/Cerone0G15} is a strengthening 
  of $\readc$ in how we add $\cfr$ edges between transactions writing  
  to the same variable.  While $\readc$ enforced a $\cfr$-ordering 
  between transactions $t_1, t_2$ writing to the same variable 
  based on the $\tto$ ordering of the corresponding read events, this 
  is strengthened in $\readat$ as follows.   
   For a transaction $t_1 \in \tran^{\wt,x}$ which is read by a read event in a transaction $t_2 \in \tran^{\rd,x}$, any transaction $t' \in \tran^{\wt,x}$  for which 
      $t' ~\trf~t_2$ or $t'~\tpo~t_2$ must be such that  $t'~\cfr~t_1$. 
   
   For all variables $x$ and all $t_1 \neq t_2 \in \tran^{\wt,x}$ such that $t_1~\trf~t_3$, $t_3 \in \tran^{\rd,x}$, if $t_2~\trf~t_3$ 
    or $t_2~\tpo~t_3$, then we have $t_2~\cfr~t_1$. 
       Define a function $\extend_{\readat}(\tau)$ which extends a trace $\tau=(\tran, \tpo, \trf)$ by 
  adding all possible $\cfr$ edges between transactions  which write on the same variable. 
  Traces violating $\readat$ exhibit a $\co \cup \cfr$ cycle in 
  $\extend_{\readat}(\tau)$, which we refer to as a $\readatcyc$. We say that $\tau \models \readat$ iff $\extend_{\readat}(\tau)$ does not contain a $\readatcyc$.  
%
%
\smallskip 
   
    \noindent{\emph{Examples}}. For the program Fig.\ref{fig:bad-app}(a), we have $t_1~\trf~t_4$ with $t_1, t_3 \in \tran^{\wt,x}$ and $t_3~\tpo~t_4$ giving $t_3~\cfr~t_1$. Likewise, we also have $t_2~\trf~t_4$ with $t_1, t_2 \in \tran^{\wt,z}$ and 
    $t_1~\rf~t_4$ (for reading into ${\tt{b}}$) giving $t_1~\cfr~t_2$ 
    resulting in $t_1~\cfr~t_2~\tpo~t_3~\cfr~t_1$ exhibiting a $\readatcyc$. Likewise, for the program in Fig.\ref{fig:bad-app}(d), 
    we have $t_3~\cfr~t_1$ (since $t_1~\trf~t_4$, $t_3~\tpo~t_4$ and $t_1, t_3 \in \tran^{\wt,x}$)
    and also $t_1~\cfr~t_2$ (since $t_2~\trf~t_5$, $t_1~\trf~t_5$ and  
        $t_1, t_2 \in \tran^{\wt,z}$) giving a $\readatcyc$.  

 
%     
%
